Delta-Complete Analysis for Bounded Reachability of Hybrid Systems

We present the framework of delta-complete analysis for bounded reachability problems of general hybrid systems. We perform bounded reachability checking through solving delta-decision problems over the reals. The techniques take into account of robustness properties of the systems under numerical perturbations. We prove that the verification problems become much more mathematically tractable in this new framework. Our implementation of the techniques, an open-source tool dReach, scales well on several highly nonlinear hybrid system models that arise in biomedical and robotics applications.

==> cav_experiments.tex <==
\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{exp_figure}
\caption{Example trajectories computed for the following models: (a) Quadcopter Control, (b) Atrial Fibrillation, (c) Electronic Oscillator.}\label{fig:exp_figure}
\end{center}
\end{figure}

Our tool {\sf dReal} implements the procedures we studied for solving
SMT formulas with ODEs. It is built on several existing packages,
including {\sf opensmt}~\cite{DBLP:conf/tacas/BruttomessoPST10} for
the general DPLL(T) framework, {\sf
  realpaver}~\cite{DBLP:journals/toms/GranvilliersB06} for ICP, and
{\sf CAPD}~\cite{capd} for computing interval-enclosures of ODEs. The
tool is open-source at~\url{http://dreal.cs.cmu.edu}. All benchmarks
and data shown here are also available on the tool website.

\newcommand{\hmodel}[2]{\href{http://dreal.cs.cmu.edu/#1}{#2}}
{\small
\begin{table}[!th]
  \centering
  \small
  \begin{tabular}{l|r|r|r|r|r|r|r|r}
    \hline
    \hline
    Benchmark    & \#Mode& \#Depth & \#ODEs & \#Vars  & Delta  & Result       & Time(s) & Trace \\
    \hline
    \hline
      AF-GOOD & 4     & 3        & 20     & 53      & 0.001     & S &  0.425    & 793K     \\
       AF-BAD & 4     & 3        & 20     & 53      & 0.001     & U &  0.074    & ---      \\
  AF-TO1-GOOD & 4     & 3        & 24     & 62      & 0.001     & S &  2.750    & 224K     \\
   AF-TO1-BAD & 4     & 3        & 24     & 62      & 0.001     & U &  5.189    & ---     \\
  AF-TO2-GOOD & 4     & 3        & 24     & 62      & 0.005     & S &  3.876    & 553K     \\
   AF-TO2-BAD & 4     & 3        & 24     & 62      & 0.001     & U &  8.857    & ---     \\
 AF-TSO1-TSO2 & 4     & 3        & 24     & 62      & 0.001     & U &  0.027    & ---     \\
       AF8-K7 & 8     & 7        & 40     & 101     & 0.001     & S & 10.478   & 3.8M      \\
      AF8-K23 & 8     & 23       & 40     & 293     & 0.001     & S & 135.29   & 11M      \\
    \hline
    \hline
    EO-K2  & 3     & 2        & 18     & 48      & 0.01    & S & 3.144    & 1.9M      \\
    EO-K11 & 3     & 11       & 99     & 174     & 0.01    & U & 0.969    & ---       \\
    \hline
    \hline
    QUAD-K1  & 2   & 1          & 34     & 89      & 0.01      & S & 2.386 &  10M \\
    QUAD-K2  & 2   & 2          & 34     & 125     & 0.01      & S & 4.971 &  13M \\
    QUAD-K3  & 4   & 3          & 68     & 161     & 0.01      & S & 13.755 & 42M \\
    QUAD-K3U & 4   & 3          & 68     & 161     & 0.01      & U & 2.846 & --- \\
    \hline
    \hline
    CT       & 2   & 2         & 10      & 41      & 0.005     & S & 345.84 & 3.1M\\
    CT       & 2   & 2         & 10      & 41      & 0.002     & S & 362.84 & 3.1M\\
    \hline
    \hline
    BB-K10 & 2     & 10       & 22     & 66      & 0.01        & S & 8.057     & 123K  \\
    BB-K20 & 2     & 20       & 42     & 126     & 0.01        & S & 39.196    & 171K  \\
    \hline
    \hline
  \end{tabular}
  \caption{\small
    \#Mode = Number of modes in the hybrid system,
    \#Depth = Unrolling depth,
    \#ODEs = Number of ODEs in the unrolled formula,
    \#Vars = Number of variables in the unrolled formula,
    Result = Bounded Model Checking Result (delta-SAT/UNSAT)
    Time = CPU time (s),
    Trace = Size of the ODE trajectory,
    AF = Atrial Filbrillation,
    EO = Electronic Oscillator,
    QUAD = Quadcopter Control,
    CT = Cancer Treatment,
    BB = Bouncing Ball with Drag.
    % TIMES = Solving time in seconds, TO = Timeout (30min), PC = Proof
    % Checked, #PA = Number of proved axioms, #SP = Number of subproblems
    % generated by proof checking, TIMEPC = Proof-checking time in seconds, #D =
    % Number of iteration depth required in proof checking
}\label{tbl:exp}
\end{table}
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "delta_reachability.tex"
%%% End:

